Does putting your emotions into words make you feel better? Measuring the minute-scale dynamics of emotions from online data

Studies of affect labeling, i.e. putting your feelings into words, indicate that it can attenuate positive and negative emotions. Here we track the evolution of individual emotions for tens of thousands of Twitter users by analyzing the emotional content of their tweets before and after they explicitly report having a strong emotion. Our results reveal how emotions and their expression evolve at the temporal resolution of one minute. While the expression of positive emotions is preceded by a short but steep increase in positive valence and followed by short decay to normal levels, negative emotions build up more slowly, followed by a sharp reversal to previous levels, matching earlier findings of the attenuating effects of affect labeling. We estimate that positive and negative emotions last approximately 1.25 and 1.5 hours from onset to evanescence. A separate analysis for male and female subjects is suggestive of possible gender-specific differences in emotional dynamics.

==> Real Mood_arXiv_final/method_diagram.tex <==
\begin{tikzpicture}

\draw [line width=0.25mm, dashed] (5.1,-1) -- (5.1,-3.75);
%\draw [line width=0.5mm] (5,-3) -- (5,-3.75);
\node[right] at (5.1,-3.5) {$t_0$: time of emotion};
%\node[right] at (5.1,-1.5) {$t_0$};

\draw[<->, line width=0.5mm] (-3,-1) -- (11,-1);
\draw[snake=ticks,segment length=1cm] (-2.9,-1) -- (10.1,-1);
\node[above] at (9.5,-1) {timeline subject $1^+$};
\node[above] at (5,-1) {"I feel \textit{+}..."};

\draw[<->, line width=0.5mm] (5,-0.25) -- ++(0,0.5) -- ++(4,0) -- ++(0,-0.5);
\node [above] at (7,0.25) {+ classification};

\draw[<->, line width=0.5mm] (-3,-2) -- (11,-2);
\draw[snake=ticks,segment length=1cm] (-2.9,-2) -- (10.1,-2);
\node[above] at (9.5,-2) {timeline subject $2^+$};

\draw[<->, line width=0.5mm](-3,-3) -- (11,-3);
\draw[snake=ticks,segment length=1cm] (-2.9,-3) -- (10.1,-3);
\node[above] at (9.5,-3) {timeline subject $3^+$};
%\node[above] at (5,-3) {"I feel \textit{great}..."};

\draw [<->, line width=0.5mm] (0.5,-3.5) -- (4.75,-3.5);
\node [below] at (2.75, -3.5) {$k$ seconds from $t_0$};

\node[above] at (-0.45,0.6) {Set of tweets $W$};
\node[above] at (-0.45,0.2) {in window};

\draw[dashed,rounded corners=4pt,line width=0.5mm]
    (0.25,-0.5) -- (-1.25,-0.5) -- (-1.25,-4) -- (0.25,-4) -- (0.25,-0.5);

\shade[color = gray,nearly transparent]
    (0.25,-0.5) -- (-1.25,-0.5) -- (-1.25,-4) -- (0.25,-4) -- (0.25,-0.5);

\draw [<->,line width=0.5mm] (-1.25,-0.20) -- (0.25, -0.20);
\node [above] at (-0.45, -0.20) {$\theta$};

\node [above] at (-0.45, -4.0) {$W_{k,\theta}$};

\draw [->,line width=0.5mm] (-0.5, -4) -- ++(0,-2.6) node [midway,fill=white]
    {$V(W_{k,\theta})$};

\node[left] at (3.3, -4.95) {VADER (V)};     
\node[left] at (3.9, -5.35) {: sentiment analysis};  
\node[left] at (3.7, -5.80) {of tweets in $W_{k,\theta}$}; 

\node [below] at (-0.5,-6.7) {$V_{k,\theta}$};

\draw [->,line width=0.5mm] (0.15,-7) -- ++(4,0) node [midway,fill=white]
    {$B(\bar{x}(V_{k,\theta}), 500)$};
    

\node [right] at (4.45, -7) 
    {$V_{k,\theta}^\prime$};
    
  
\node [right] at (0, -7.65) 
    {bootstrapping $\bar{x}(V_{k,\theta}) \times 500$}; 
    
\draw [->, line width=0.5mm] (5.45, -7) -- ++(0.45,0);

 
%%%% DRAW NORMAL DISTRIBUTION

% define normal distribution function 'normaltwo'
    \def\normaltwo{\x+\sx,{2*1/exp(((\x-3)^2)/1)+\sy}}

% define normal distribution function 'normaltwo'
    \def\normaltwoa{\x+\sx+0.27,{2*1/exp(((\x-3)^2)/1.2)+\sy+0.35}}

% define normal distribution function 'normaltwo'
    \def\normaltwob{\x+\sx+0.5,{2*1/exp(((\x-3)^2)/0.7)+\sy+0.74}}
    
% define normal distribution function 'normaltwo'
    \def\normaltwoc{\x+\sx+0.69,{2*1/exp(((\x-2.8)^2)/0.6)+\sy+1}}

% starting x and y
    \def\sx{5.75}
    \def\sy{-7.0}

% input x and y parameters
    \def\y{4.25}
    \def\x{1.75}
    \def\m{3}
 
% this line calculates f(y)
    \def\fy{2*1/exp(((\x-3)^2)/1)}
    \def\fx{2*1/exp(((\x-3)^2)/1)}
    \def\fm{2*1/exp(((\x-3)^2)/1)}
    
% Shade orange area underneath curve.
%    \fill [fill=orange!60] ({\x+\sx},0+\sy) -- 
%        plot[domain={\x}+\sx:{\y}+\sy] (\normaltwo) -- ({\y}+\sx,0+\sy) -- cycle;
 
% Draw and label normal distribution function
    \draw[line width=0.5mm, color=blue,domain=1:5] plot (\normaltwo) node[right] {};
    \draw[line width=0.4mm, color=blue,domain=1:5] plot (\normaltwoa) node[right] {};
    \draw[line width=0.3mm, color=blue,domain=1:5] plot (\normaltwob) node[right] {};
    \draw[line width=0.3mm, color=blue,domain=1:5] plot (\normaltwoc) node[right] {};
    
% Add dashed line dropping down from normal.
    \draw[dashed] ({\y+\sx},{\fy+\sy}) -- ({\y+\sx},0+\sy) node[below] {$5p$};
    \draw[dashed] ({\x+\sx},{\fx+\sy}) -- ({\x+\sx},0+\sy) node[below] {$95p$};
    \draw[dashed] ({\m+\sx},{\fm+\sy}) -- ({\m+\sx},0+\sy) node[below] {$50p$};
    
    \draw[<->, dashed] ({\m+\sx-1},{\fm+\sy}) -- ({\m+\sx+1},{\fm+\sy})
        node[midway,fill=white] {$CI$};
 
% Optional: Add axis labels
    \draw (1+\sx,2+\sy) node[left] {$P(V_{k,\theta}^\prime)$};
    \draw (5.5+\sx,\sy-0.1) node[below] {$V_{k,\theta}^\prime$};
    \draw (2.4+\sx,2.8+\sy) node[below] {$k$};
 
% Optional: Add axes
    \draw[->,line width=0.5mm] (\sx+1,\sy) -- (5.5+\sx,\sy) node[right] {};
    \draw[->,line width=0.5mm] (\sx+1,\sy) -- ++(0,+2.5) node[above] {};
    \draw[->,line width=0.5mm] (\sx+1,\sy) -- (\sx+2.7,\sy+2.40) node[above] {};
    
% add t_0 line
   \draw[dashed] (\sx+2.2,\sy+1.6) -- ++(3.0,0) node[right] {$t_0$};
  
\end{tikzpicture}

==> method_diagram.tex <==
\begin{tikzpicture}

\draw [line width=0.25mm, dashed] (5.1,-1) -- (5.1,-3.75);
%\draw [line width=0.5mm] (5,-3) -- (5,-3.75);
\node[right] at (5.1,-3.5) {$t_0$: time of emotion};
%\node[right] at (5.1,-1.5) {$t_0$};

\draw[<->, line width=0.5mm] (-3,-1) -- (11,-1);
\draw[snake=ticks,segment length=1cm] (-2.9,-1) -- (10.1,-1);
\node[above] at (9.5,-1) {timeline subject $1^+$};
\node[above] at (5,-1) {"I feel \textit{+}..."};

\draw[<->, line width=0.5mm] (5,-0.25) -- ++(0,0.5) -- ++(4,0) -- ++(0,-0.5);
\node [above] at (7,0.25) {+ classification};

\draw[<->, line width=0.5mm] (-3,-2) -- (11,-2);
\draw[snake=ticks,segment length=1cm] (-2.9,-2) -- (10.1,-2);
\node[above] at (9.5,-2) {timeline subject $2^+$};

\draw[<->, line width=0.5mm](-3,-3) -- (11,-3);
\draw[snake=ticks,segment length=1cm] (-2.9,-3) -- (10.1,-3);
\node[above] at (9.5,-3) {timeline subject $3^+$};
%\node[above] at (5,-3) {"I feel \textit{great}..."};

\draw [<->, line width=0.5mm] (0.5,-3.5) -- (4.75,-3.5);
\node [below] at (2.75, -3.5) {$k$ seconds from $t_0$};

\node[above] at (-0.45,0.6) {Set of tweets $W$};
\node[above] at (-0.45,0.2) {in window};

\draw[dashed,rounded corners=4pt,line width=0.5mm]
    (0.25,-0.5) -- (-1.25,-0.5) -- (-1.25,-4) -- (0.25,-4) -- (0.25,-0.5);

\shade[color = gray,nearly transparent]
    (0.25,-0.5) -- (-1.25,-0.5) -- (-1.25,-4) -- (0.25,-4) -- (0.25,-0.5);

\draw [<->,line width=0.5mm] (-1.25,-0.20) -- (0.25, -0.20);
\node [above] at (-0.45, -0.20) {$\theta$};

\node [above] at (-0.45, -4.0) {$W_{k,\theta}$};

\draw [->,line width=0.5mm] (-0.5, -4) -- ++(0,-2.6) node [midway,fill=white]
    {$V(W_{k,\theta})$};

\node[left] at (3.3, -4.95) {VADER (V)};     
\node[left] at (3.9, -5.35) {: sentiment analysis};  
\node[left] at (3.7, -5.80) {of tweets in $W_{k,\theta}$}; 

\node [below] at (-0.5,-6.7) {$V_{k,\theta}$};

\draw [->,line width=0.5mm] (0.15,-7) -- ++(4,0) node [midway,fill=white]
    {$B(\bar{x}(V_{k,\theta}), 500)$};
    

\node [right] at (4.45, -7) 
    {$V_{k,\theta}^\prime$};
    
  
\node [right] at (0, -7.65) 
    {bootstrapping $\bar{x}(V_{k,\theta}) \times 500$}; 
    
\draw [->, line width=0.5mm] (5.45, -7) -- ++(0.45,0);

 
%%%% DRAW NORMAL DISTRIBUTION

% define normal distribution function 'normaltwo'
    \def\normaltwo{\x+\sx,{2*1/exp(((\x-3)^2)/1)+\sy}}

% define normal distribution function 'normaltwo'
    \def\normaltwoa{\x+\sx+0.27,{2*1/exp(((\x-3)^2)/1.2)+\sy+0.35}}

% define normal distribution function 'normaltwo'
    \def\normaltwob{\x+\sx+0.5,{2*1/exp(((\x-3)^2)/0.7)+\sy+0.74}}
    
% define normal distribution function 'normaltwo'
    \def\normaltwoc{\x+\sx+0.69,{2*1/exp(((\x-2.8)^2)/0.6)+\sy+1}}

% starting x and y
    \def\sx{5.75}
    \def\sy{-7.0}

% input x and y parameters
    \def\y{4.25}
    \def\x{1.75}
    \def\m{3}
 
% this line calculates f(y)
    \def\fy{2*1/exp(((\x-3)^2)/1)}
    \def\fx{2*1/exp(((\x-3)^2)/1)}
    \def\fm{2*1/exp(((\x-3)^2)/1)}
    
% Shade orange area underneath curve.
%    \fill [fill=orange!60] ({\x+\sx},0+\sy) -- 
%        plot[domain={\x}+\sx:{\y}+\sy] (\normaltwo) -- ({\y}+\sx,0+\sy) -- cycle;
 
% Draw and label normal distribution function
    \draw[line width=0.5mm, color=blue,domain=1:5] plot (\normaltwo) node[right] {};
    \draw[line width=0.4mm, color=blue,domain=1:5] plot (\normaltwoa) node[right] {};
    \draw[line width=0.3mm, color=blue,domain=1:5] plot (\normaltwob) node[right] {};
    \draw[line width=0.3mm, color=blue,domain=1:5] plot (\normaltwoc) node[right] {};
    
% Add dashed line dropping down from normal.
    \draw[dashed] ({\y+\sx},{\fy+\sy}) -- ({\y+\sx},0+\sy) node[below] {$5p$};
    \draw[dashed] ({\x+\sx},{\fx+\sy}) -- ({\x+\sx},0+\sy) node[below] {$95p$};
    \draw[dashed] ({\m+\sx},{\fm+\sy}) -- ({\m+\sx},0+\sy) node[below] {$50p$};
    
    \draw[<->, dashed] ({\m+\sx-1},{\fm+\sy}) -- ({\m+\sx+1},{\fm+\sy})
        node[midway,fill=white] {$CI$};
 
% Optional: Add axis labels
    \draw (1+\sx,2+\sy) node[left] {$P(V_{k,\theta}^\prime)$};
    \draw (5.5+\sx,\sy-0.1) node[below] {$V_{k,\theta}^\prime$};
    \draw (2.4+\sx,2.8+\sy) node[below] {$k$};
 
% Optional: Add axes
    \draw[->,line width=0.5mm] (\sx+1,\sy) -- (5.5+\sx,\sy) node[right] {};
    \draw[->,line width=0.5mm] (\sx+1,\sy) -- ++(0,+2.5) node[above] {};
    \draw[->,line width=0.5mm] (\sx+1,\sy) -- (\sx+2.7,\sy+2.40) node[above] {};
    
% add t_0 line
   \draw[dashed] (\sx+2.2,\sy+1.6) -- ++(3.0,0) node[right] {$t_0$};
  
\end{tikzpicture}
